Observation of the annihilation decay mode $B^{0}\to K^{+}K^{-}$

A search for the $B^{0}\to K^{+}K^{-}$ decay is performed using $pp$-collision data collected by LHCb. The data set corresponds to integrated luminosities of 1 and 2 fb$^{-1}$ at center-of-mass energies of 7 and 8 TeV, respectively. This decay is observed for the first time, with a significance of more than five standard deviations. The analysis also results in an improved measurement of the branching fraction for the $B_s^0\to \pi^+\pi^-$ decay. The measured branching fractions are $BR(B^0\to K^+K^-) = (7.80 \pm 1.27 \pm 0.81 \pm 0.21) \times 10^{-8}$ and $BR(B_s^0\to\pi^+\pi^-) = (6.91 \pm 0.54 \pm 0.63 \pm 0.19 \pm 0.40) \times 10^{-7}$. The first uncertainty is statistical, the second is systematic, the third is due to the uncertainty on the $B^0\to K^+\pi^-$ branching fraction used as a normalization. For the $B_s^0$ mode, the fourth accounts for the uncertainty on the ratio of the probabilities for $b$ quarks to hadronize into $B_s^0$ and $B^0$ mesons.

==> LHCb_Authorship_flat_arXiv_13-Jul-2016.tex <==
LHCb collaboration: 
R. Aaij,
B. Adeva,
M. Adinolfi,
Z. Ajaltouni,
S. Akar,
J. Albrecht,
F. Alessio,
M. Alexander,
S. Ali,
G. Alkhazov,
P. Alvarez Cartelle,
A.A. Alves Jr,
S. Amato,
S. Amerio,
Y. Amhis,
L. An,
L. Anderlini,
G. Andreassi,
M. Andreotti,
J.E. Andrews,
R.B. Appleby,
F. Archilli,
P. d'Argent,
J. Arnau Romeu,
A. Artamonov,
M. Artuso,
E. Aslanides,
G. Auriemma,
M. Baalouch,
I. Babuschkin,
S. Bachmann,
J.J. Back,
A. Badalov,
C. Baesso,
S. Baker,
W. Baldini,
R.J. Barlow,
C. Barschel,
S. Barsuk,
W. Barter,
M. Baszczyk,
V. Batozskaya,
B. Batsukh,
V. Battista,
A. Bay,
L. Beaucourt,
J. Beddow,
F. Bedeschi,
I. Bediaga,
L.J. Bel,
V. Bellee,
N. Belloli,
K. Belous,
I. Belyaev,
E. Ben-Haim,
G. Bencivenni,
S. Benson,
J. Benton,
A. Berezhnoy,
R. Bernet,
A. Bertolin,
F. Betti,
M.-O. Bettler,
M. van Beuzekom,
Ia. Bezshyiko,
S. Bifani,
P. Billoir,
T. Bird,
A. Birnkraut,
A. Bitadze,
A. Bizzeti,
T. Blake,
F. Blanc,
J. Blouw,
S. Blusk,
V. Bocci,
T. Boettcher,
A. Bondar,
N. Bondar,
W. Bonivento,
A. Borgheresi,
S. Borghi,
M. Borisyak,
M. Borsato,
F. Bossu,
M. Boubdir,
T.J.V. Bowcock,
E. Bowen,
C. Bozzi,
S. Braun,
M. Britsch,
T. Britton,
J. Brodzicka,
E. Buchanan,
C. Burr,
A. Bursche,
J. Buytaert,
S. Cadeddu,
R. Calabrese,
M. Calvi,
M. Calvo Gomez,
A. Camboni,
P. Campana,
D. Campora Perez,
D.H. Campora Perez,
L. Capriotti,
A. Carbone,
G. Carboni,
R. Cardinale,
A. Cardini,
P. Carniti,
L. Carson,
K. Carvalho Akiba,
G. Casse,
L. Cassina,
L. Castillo Garcia,
M. Cattaneo,
Ch. Cauet,
G. Cavallero,
R. Cenci,
M. Charles,
Ph. Charpentier,
G. Chatzikonstantinidis,
M. Chefdeville,
S. Chen,
S.-F. Cheung,
V. Chobanova,
M. Chrzaszcz,
X. Cid Vidal,
G. Ciezarek,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
V. Coco,
J. Cogan,
E. Cogneras,
V. Cogoni,
L. Cojocariu,
G. Collazuol,
P. Collins,
A. Comerma-Montells,
A. Contu,
A. Cook,
G. Coombs,
S. Coquereau,
G. Corti,
M. Corvo,
C.M. Costa Sobral,
B. Couturier,
G.A. Cowan,
D.C. Craik,
A. Crocombe,
M. Cruz Torres,
S. Cunliffe,
R. Currie,
C. D'Ambrosio,
F. Da Cunha Marinho,
E. Dall'Occo,
J. Dalseno,
P.N.Y. David,
A. Davis,
O. De Aguiar Francisco,
K. De Bruyn,
S. De Capua,
M. De Cian,
J.M. De Miranda,
L. De Paula,
M. De Serio,
P. De Simone,
C.-T. Dean,
D. Decamp,
M. Deckenhoff,
L. Del Buono,
M. Demmer,
D. Derkach,
O. Deschamps,
F. Dettori,
B. Dey,
A. Di Canto,
H. Dijkstra,
F. Dordei,
M. Dorigo,
A. Dosil Su{\'a}rez,
A. Dovbnya,
K. Dreimanis,
L. Dufour,
G. Dujany,
K. Dungs,
P. Durante,
R. Dzhelyadin,
A. Dziurda,
A. Dzyuba,
N. D{\'e}l{\'e}age,
S. Easo,
M. Ebert,
U. Egede,
V. Egorychev,
S. Eidelman,
S. Eisenhardt,
U. Eitschberger,
R. Ekelhof,
L. Eklund,
Ch. Elsasser,
S. Ely,
S. Esen,
H.M. Evans,
T. Evans,
A. Falabella,
N. Farley,
S. Farry,
R. Fay,
D. Fazzini,
D. Ferguson,
V. Fernandez Albor,
A. Fernandez Prieto,
F. Ferrari,
F. Ferreira Rodrigues,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiore,
M. Fiorini,
M. Firlej,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
K. Fohl,
M. Fontana,
F. Fontanelli,
D.C. Forshaw,
R. Forty,
V. Franco Lima,
M. Frank,
C. Frei,
J. Fu,
E. Furfaro,
C. F{\"a}rber,
A. Gallas Torreira,
D. Galli,
S. Gallorini,
S. Gambetta,
M. Gandelman,
P. Gandini,
Y. Gao,
L.M. Garcia Martin,
J. Garc{\'\i}a Pardi{\~n}as,
J. Garra Tico,
L. Garrido,
P.J. Garsed,
D. Gascon,
C. Gaspar,
L. Gavardi,
G. Gazzoni,
D. Gerick,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
Ph. Ghez,
S. Gian{\`\i},
V. Gibson,
O.G. Girard,
L. Giubega,
K. Gizdov,
V.V. Gligorov,
D. Golubkov,
A. Golutvin,
A. Gomes,
I.V. Gorelov,
C. Gotti,
M. Grabalosa G{\'a}ndara,
R. Graciani Diaz,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
G. Graziani,
A. Grecu,
P. Griffith,
L. Grillo,
B.R. Gruberg Cazon,
O. Gr{\"u}nberg,
E. Gushchin,
Yu. Guz,
T. Gys,
C. G{\"o}bel,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
S.C. Haines,
S. Hall,
B. Hamilton,
X. Han,
S. Hansmann-Menzemer,
N. Harnew,
S.T. Harnew,
J. Harrison,
M. Hatch,
J. He,
T. Head,
A. Heister,
K. Hennessy,
P. Henrard,
L. Henry,
J.A. Hernando Morata,
E. van Herwijnen,
M. He{\ss},
A. Hicheur,
D. Hill,
C. Hombach,
H. Hopchev,
W. Hulsbergen,
T. Humair,
M. Hushchyn,
N. Hussain,
D. Hutchcroft,
M. Idzik,
P. Ilten,
R. Jacobsson,
A. Jaeger,
J. Jalocha,
E. Jans,
A. Jawahery,
F. Jiang,
M. John,
D. Johnson,
C.R. Jones,
C. Joram,
B. Jost,
N. Jurik,
S. Kandybei,
W. Kanso,
M. Karacson,
J.M. Kariuki,
S. Karodia,
M. Kecke,
M. Kelsey,
I.R. Kenyon,
M. Kenzie,
T. Ketel,
E. Khairullin,
B. Khanji,
C. Khurewathanakul,
T. Kirn,
S. Klaver,
K. Klimaszewski,
S. Koliiev,
M. Kolpin,
I. Komarov,
R.F. Koopman,
P. Koppenburg,
A. Kosmyntseva,
A. Kozachuk,
M. Kozeiha,
L. Kravchuk,
K. Kreplin,
M. Kreps,
P. Krokovny,
F. Kruse,
W. Krzemien,
W. Kucewicz,
M. Kucharczyk,
V. Kudryavtsev,
A.K. Kuonen,
K. Kurek,
T. Kvaratskheliya,
D. Lacarrere,
G. Lafferty,
A. Lai,
D. Lambert,
G. Lanfranchi,
C. Langenbruch,
T. Latham,
C. Lazzeroni,
R. Le Gac,
J. van Leerdam,
J.-P. Lees,
A. Leflat,
J. Lefran{\c{c}}ois,
R. Lef{\`e}vre,
F. Lemaitre,
E. Lemos Cid,
O. Leroy,
T. Lesiak,
B. Leverington,
Y. Li,
T. Likhomanenko,
R. Lindner,
C. Linn,
F. Lionetto,
B. Liu,
X. Liu,
D. Loh,
I. Longstaff,
J.H. Lopes,
D. Lucchesi,
M. Lucio Martinez,
H. Luo,
A. Lupato,
E. Luppi,
O. Lupton,
A. Lusiani,
X. Lyu,
F. Machefert,
F. Maciuc,
O. Maev,
K. Maguire,
S. Malde,
A. Malinin,
T. Maltsev,
G. Manca,
G. Mancinelli,
P. Manning,
J. Maratas,
J.F. Marchand,
U. Marconi,
C. Marin Benito,
P. Marino,
J. Marks,
G. Martellotti,
M. Martin,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
D. Martins Tostes,
L.M. Massacrier,
A. Massafferri,
R. Matev,
A. Mathad,
Z. Mathe,
C. Matteuzzi,
A. Mauri,
B. Maurin,
A. Mazurov,
M. McCann,
J. McCarthy,
A. McNab,
R. McNulty,
B. Meadows,
F. Meier,
M. Meissner,
D. Melnychuk,
M. Merk,
A. Merli,
E. Michielin,
D.A. Milanes,
M.-N. Minard,
D.S. Mitzel,
A. Mogini,
J. Molina Rodriguez,
I.A. Monroy,
S. Monteil,
M. Morandin,
P. Morawski,
A. Mord{\`a},
M.J. Morello,
J. Moron,
A.B. Morris,
R. Mountain,
F. Muheim,
M. Mulder,
M. Mussini,
D. M{\"u}ller,
J. M{\"u}ller,
K. M{\"u}ller,
V. M{\"u}ller,
P. Naik,
T. Nakada,
R. Nandakumar,
A. Nandi,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
M. Neuner,
A.D. Nguyen,
C. Nguyen-Mau,
S. Nieswand,
R. Niet,
N. Nikitin,
T. Nikodem,
A. Novoselov,
D.P. O'Hanlon,
A. Oblakowska-Mucha,
V. Obraztsov,
S. Ogilvy,
R. Oldeman,
C.J.G. Onderwater,
J.M. Otalora Goicochea,
A. Otto,
P. Owen,
A. Oyanguren,
P.R. Pais,
A. Palano,
F. Palombo,
M. Palutan,
J. Panman,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
W. Parker,
C. Parkes,
G. Passaleva,
A. Pastore,
G.D. Patel,
M. Patel,
C. Patrignani,
A. Pearce,
A. Pellegrino,
G. Penso,
M. Pepe Altarelli,
S. Perazzini,
P. Perret,
L. Pescatore,
K. Petridis,
A. Petrolini,
A. Petrov,
M. Petruzzo,
E. Picatoste Olloqui,
B. Pietrzyk,
M. Pikies,
D. Pinci,
A. Pistone,
A. Piucci,
S. Playfer,
M. Plo Casasus,
T. Poikela,
F. Polci,
A. Poluektov,
I. Polyakov,
E. Polycarpo,
G.J. Pomery,
A. Popov,
D. Popov,
B. Popovici,
S. Poslavskii,
C. Potterat,
E. Price,
J.D. Price,
J. Prisciandaro,
A. Pritchard,
C. Prouve,
V. Pugatch,
A. Puig Navarro,
G. Punzi,
W. Qian,
R. Quagliani,
B. Rachwal,
J.H. Rademacker,
M. Rama,
M. Ramos Pernas,
M.S. Rangel,
I. Raniuk,
G. Raven,
F. Redi,
S. Reichert,
A.C. dos Reis,
C. Remon Alepuz,
V. Renaudin,
S. Ricciardi,
S. Richards,
M. Rihl,
K. Rinnert,
V. Rives Molina,
P. Robbe,
A.B. Rodrigues,
E. Rodrigues,
J.A. Rodriguez Lopez,
P. Rodriguez Perez,
A. Rogozhnikov,
S. Roiser,
A. Rollings,
V. Romanovskiy,
A. Romero Vidal,
J.W. Ronayne,
M. Rotondo,
M.S. Rudolph,
T. Ruf,
P. Ruiz Valls,
J.J. Saborido Silva,
E. Sadykhov,
N. Sagidova,
B. Saitta,
V. Salustino Guimaraes,
C. Sanchez Mayordomo,
B. Sanmartin Sedes,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
E. Santovetti,
A. Sarti,
C. Satriano,
A. Satta,
D.M. Saunders,
D. Savrina,
S. Schael,
M. Schellenberg,
M. Schiller,
H. Schindler,
M. Schlupp,
M. Schmelling,
T. Schmelzer,
B. Schmidt,
O. Schneider,
A. Schopper,
K. Schubert,
M. Schubiger,
M.-H. Schune,
R. Schwemmer,
B. Sciascia,
A. Sciubba,
A. Semennikov,
A. Sergi,
N. Serra,
J. Serrano,
L. Sestini,
P. Seyfert,
M. Shapkin,
I. Shapoval,
Y. Shcheglov,
T. Shears,
L. Shekhtman,
V. Shevchenko,
A. Shires,
B.G. Siddi,
R. Silva Coutinho,
L. Silva de Oliveira,
G. Simi,
S. Simone,
M. Sirendi,
N. Skidmore,
T. Skwarnicki,
E. Smith,
I.T. Smith,
J. Smith,
M. Smith,
H. Snoek,
M.D. Sokoloff,
F.J.P. Soler,
B. Souza De Paula,
B. Spaan,
P. Spradlin,
S. Sridharan,
F. Stagni,
M. Stahl,
S. Stahl,
P. Stefko,
S. Stefkova,
O. Steinkamp,
S. Stemmle,
O. Stenyakin,
S. Stevenson,
S. Stoica,
S. Stone,
B. Storaci,
S. Stracka,
M. Straticiuc,
U. Straumann,
L. Sun,
W. Sutcliffe,
K. Swientek,
V. Syropoulos,
M. Szczekowski,
T. Szumlak,
S. T'Jampens,
A. Tayduganov,
T. Tekampe,
G. Tellarini,
F. Teubert,
E. Thomas,
J. van Tilburg,
M.J. Tilley,
V. Tisserand,
M. Tobin,
S. Tolk,
L. Tomassetti,
D. Tonelli,
S. Topp-Joergensen,
F. Toriello,
E. Tournefier,
S. Tourneur,
K. Trabelsi,
M. Traill,
M.T. Tran,
M. Tresch,
A. Trisovic,
A. Tsaregorodtsev,
P. Tsopelas,
A. Tully,
N. Tuning,
A. Ukleja,
A. Ustyuzhanin,
U. Uwer,
C. Vacca,
V. Vagnoni,
A. Valassi,
S. Valat,
G. Valenti,
A. Vallier,
R. Vazquez Gomez,
P. Vazquez Regueiro,
S. Vecchi,
M. van Veghel,
J.J. Velthuis,
M. Veltri,
G. Veneziano,
A. Venkateswaran,
M. Vernet,
M. Vesterinen,
B. Viaud,
D.  Vieira,
M. Vieites Diaz,
X. Vilasis-Cardona,
V. Volkov,
A. Vollhardt,
B. Voneki,
A. Vorobyev,
V. Vorobyev,
C. Vo{\ss},
J.A. de Vries,
C. V{\'a}zquez Sierra,
R. Waldi,
C. Wallace,
R. Wallace,
J. Walsh,
J. Wang,
D.R. Ward,
H.M. Wark,
N.K. Watson,
D. Websdale,
A. Weiden,
M. Whitehead,
J. Wicht,
G. Wilkinson,
M. Wilkinson,
M. Williams,
M.P. Williams,
M. Williams,
T. Williams,
F.F. Wilson,
J. Wimberley,
J. Wishahi,
W. Wislicki,
M. Witek,
G. Wormser,
S.A. Wotton,
K. Wraight,
S. Wright,
K. Wyllie,
Y. Xie,
Z. Xing,
Z. Xu,
Z. Yang,
H. Yin,
J. Yu,
X. Yuan,
O. Yushchenko,
K.A. Zarebski,
M. Zavertyaev,
L. Zhang,
Y. Zhang,
Y. Zhang,
A. Zhelezov,
Y. Zheng,
A. Zhokhov,
X. Zhu,
V. Zhukov,
S. Zucchelli
